Some Targets Are Harder to Identify than Others: Quantifying the Target-dependent Membership Leakage

In a Membership Inference (MI) game, an attacker tries to infer whether a target point was included or not in the input of an algorithm. Existing works show that some target points are easier to identify, while others are harder. This paper explains the target-dependent hardness of membership attacks by studying the powers of the optimal attacks in a fixed-target MI game. We characterise the optimal advantage and trade-off functions of attacks against the empirical mean in terms of the Mahalanobis distance between the target point and the data-generating distribution. We further derive the impacts of two privacy defences, i.e. adding Gaussian noise and sub-sampling, and that of target misspecification on optimal attacks. As by-products of our novel analysis of the Likelihood Ratio (LR) test, we provide a new covariance attack which generalises and improves the scalar product attack. Also, we propose a new optimal canary-choosing strategy for auditing privacy in the white-box federated learning setting. Our experiments validate that the Mahalanobis score explains the hardness of fixed-target MI games.

==> sections/related_work.tex <==
\subsection{Related Works}
Main question:
Explain and quantify the per-example hardness in membership inference: Why some examples are harder to attack than others?

Main application: 
Designing better canaries for privacy auditing: a canary is an example that is easy to attack,
Also designing better attacks that adapt to the hardness of the example to attack.

Main contributions:
Studying the Per-example membership setting, consequences of Pearson lemma, defining Per-example membership leakage notion

Average-example setting fully introduced in:
"Samuel Yeom, Irene Giacomelli, Matt Fredrikson, and Somesh Jha. Privacy risk in machine learning: Analyzing the connection to overfitting" = Average-example setting.

Per-example membership problem was also introduced in: ...

Enhanced membership inference attacks against machine learning models: Definition 3.3 (Membership inference game for a fixed record) "Similar inference games that only target (a)
specific record(s) are used in previous works for pragmatic, high-
precision membership inference attacks on a subset of vulnerable
records [17, 18], and for estimating privacy risks of data records in different subgroups [4]."

Membership attacks from first principle: using per-example hardness scores + LR test, assymption: parametric modeling  Sablayrolles et al. (2019)'s assymption and refs [37,56, 68, 69] there in .


Main mechanism we analyse: exact empirical mean. We quantify the exact asymptotic per-example leakage and show that it depends on the Mahalanobis distance of the example, new proof using the Hedgeworth expansion in the CLT, fully characterise the power type 1/type 2 error profile.

Related work: 
Tracing/Genomic litt:
- Homer, first attack on exact empirical mean
- Sriram (only for bernoulli + average-example setting not per-example one), 
- Dwork (scalar product attack, only needs one reference point), 

Machine learning litt:
- "Samuel Yeom, Irene Giacomelli, Matt Fredrikson, and Somesh Jha. Privacy risk in machine learning: Analyzing the connection to overfitting" = average-record, simple loss-based attacks.
- Gaussian Membership Privacy (proof assumes gaussian distribution, bad use of CLT), 
- "Parameters or Privacy: A Provable Tradeoff Between
Overparameterization and Membership Inference", theoretical analysis of LR test for linear regression (average example setting) 

==> also we provide an approximate "practical" LR test, gives better understanding of the relation between Sriram's LR attack and Dwork's scalar product attack.

Different variations of the setting: 
- effect of adding gaussian noise, 
- effect of subsampling, 
- misspecification and attacking similar points.
- relation to DP

Auditing and canaries:
- White box = directly using our insights from exact empirical mean, since one step of SGD is just an empirical mean of loss gradient ==> using Mahalanobis distance based functions to compute scores and to find canaries
- Black-box = gereralisation to empirical risk minimization using z-estimators asymptotic properties: asymp. dist of a z-estimator == empirical mean of influence function ==> using influence based functions to compute scores and to find canaries 

Main Related works:
Privacy Auditing with One (1) Training Run and refs in section 3 related works therein.








